DeVIT: Low-Power Vision Transformer Acceleration Using Delta Computation

The emergence of transformer-based deep learning models has brought unprecedented performance across various domains, particularly in natural language processing and computer vision. However, deploying these models, especially on resource-constrained devices, poses significant challenges due to their high computational complexity and large memory size and bandwidth requirements. This complexity has led researchers to use low-bit model weights to reduce memory usage and improve efficiency. In addition to reducing processing and memory demands, quantization introduces another useful property: value locality, where the extremely large number of parameters are restricted to a limited range of values. To fully take advantage of this locality, this paper presents DeVIT, an acceleration method for vision transformers that leverages differential computation to enable multiplier-less matrix multiplication.

==> sections/5_DeVIT_Arch.tex <==
% !TeX root = ../Main.tex
% This file is a section fragment; compile Main.tex rather than this file.
The proposed architecture of DeVIT, depicted in Fig.~\ref{fig:DeVIT_Unit}, comprises three primary components: an input buffer, a processing unit, and an index management subsystem. The processing unit operates as a Shift-Add-Accumulator, receiving two inputs---the activation value and the encoded weight value---to generate partial products. To ensure the proper alignment of encoded weights with their original positions, index addresses are pre-stored offline in an index buffer. During execution, the controller dynamically retrieves the actual indices from this buffer and associates them with the partial results produced by the processing unit. This controller, which can be implemented using a multiplexer or an on-chip interconnect such as a CLOS network, guarantees accurate mapping between the encoded values and their corresponding output locations. The computed partial products are then written to the output buffer at the specified locations, as determined by the resolved indices, thus maintaining the correctness and consistency of the data flow.

\noindent In this architecture, accumulation takes place simultaneously in both the register within the processing unit---referred to as the DeVIT unit---and the output buffer. During the subsequent cycle, the register accumulates the next element of the encoded weight vector for the current row using the same activation input, thereby preparing the next contribution to the designated location in the output buffer. Once a given activation input has been processed across all elements of an encoded weight vector, the output buffer contains the initial partial products. Concurrently, the output buffer continues to be updated as the DeVIT unit processes the following activation input alongside the subsequent row of encoded weight values, generating additional partial products. This parallel accumulation mechanism facilitates efficient pipelined execution throughout the matrix, minimizing idle cycles within the DeVIT unit.

\noindent The weights are pre-encoded offline by quantizing the differences between consecutive sorted weights to the nearest power of two. The corresponding exponents are then stored as the encoded representation.

\noindent During execution, the input activation is adjusted based on the stored exponent in each cycle. In subsequent cycles, this activation is combined with the previously generated partial sums.


% IEEE-friendly LaTeX (pdfLaTeX-safe). Assumes \usepackage{amsmath}.
\noindent To tackle the challenges associated with buffer capacity and power efficiency in neural network computations, we implement a strategic weight-matrix management scheme. When the size of the output buffer corresponds to the encoded weight value, a substantial number of on-the-fly partial products are produced, resulting in increased power consumption.

\noindent In this strategy, we partition the weight matrices into appropriately sized blocks before applying DeVIT. This reduces the overhead associated with generating partial products and alleviates issues related to power and buffer limitations. The advantages of this partitioning strategy include:
\begin{enumerate}
  \item Decreased buffer size, as each partitioned block is smaller than the original matrix.
  \item Potentially lower power consumption due to the reduced buffer size.
  \item Enhanced efficiency in applying the delta method and input-stationary approach to these smaller blocks.
  \item Improved flexibility for processing, allowing for the possibility of parallel computation across different blocks.
\end{enumerate}

\noindent By utilizing this partitioning technique in conjunction with the DeVIT unit, we can achieve a more favorable balance between performance and resource utilization.

\noindent In our analysis, we assessed the weights of the ViT-B/16 model by dividing them into blocks and calculating the frequency of the delta distribution across its 12 layers. We accomplished this by averaging the frequency of delta values within each block, then averaging those results across all blocks, and finally averaging across the 12 layers.

\noindent The diagram presented in Fig.~\ref{fig:DeVIT_Unit_partitioned} illustrates our process: we first partition the weights, then sort and encode them in delta format. We apply DeVIT to generate the partial products, which are subsequently stored in an output buffer. Finally, we restore the elements of each column to their correct positions and accumulate them. Through this partitioning process, we effectively achieve both input-stationary and output-stationary mechanisms, as the first input must be read to facilitate the subsequent partitions.




% Adding the image in one column
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{./visio-unit.pdf}
    \caption{The DeltaViT unit.}
    \label{fig:DeVIT_Unit}
\end{figure}



% Adding the image in one column
\begin{figure}[h!]
    \centering
    \includegraphics[width=\columnwidth]{./visio-unit-partitioned.pdf}
    \caption{The architecture of partitioned producing partial products with differentiated weights (deltas).}
    \label{fig:DeVIT_Unit_partitioned}
\end{figure}

